Monotone Rewritability and the Analysis of Queries, Views, and Rules

We study the interaction of views, queries, and background knowledge in the form of existential rules. The motivating questions concern monotonic determinacy of a query using views w.r.t. rules, which refers to the ability to recover the query answer from the views via a monotone function. We study the decidability of monotonic determinacy, and compare with variations that require the ``recovery function'' to be in a well-known monotone query language, such as conjunctive queries or Datalog. Surprisingly, we find that even in the presence of basic existential rules, the borderline between well-behaved and badly-behaved answerability differs radically from the unconstrained case. In order to understand this boundary, we require new results concerning entailment problems involving views and rules.

==> app-frontierdecide.tex <==
\myparagraph{Proof details for Theorem \ref{thm:frontieronecqcq}}
Recall the statement of the theorem:


\medskip

Suppose $\Sigma$ ranges over frontier-one TGDs.
Then monotonic determinacy of CQ  $Q$ over CQ views $\views$ relative
to $\Sigma$ is decidable.

\medskip

We recall the proof from the body.
We can apply Theorem \ref{thm:rewritefrontieronemdl} to get $R_1$ a  MDL $\certainanswerrewriting$ of $Q$ with respect to $\Sigma$.
We can then get an extensionally-connected Datalog query $R_2$ \michael{Use an argument that we can get an MDL query!} that is a $\certainanswerrewriting$ of  $R_1$ with respect to $\backview_\views$.  %\michael{Check that we are applying this correctly}
Success of the process in Figure \ref{alg:query-mondet-constraints} is then captured by
entailment of $R_2$ by $Q$ with respect to $\Sigma$.
But we can argue that such an entailment is decidable.


==> app-highlyundecidable.tex <==
%\subsection*{Beyond undecidability for monotonic determinacy for Datalog with constraints} \label{sec:highly}
Let us consider monotonic determinacy of  Datalog queries and Datalog views with respect to first-order background knowledge
over \emph{finite instances}.  When this fails, we will always have finite counterexamples,  by definition. A counterexample
consists of two instances $\inst_1$ and $\inst_2$ satisfying the rules, where the view image in $\inst_1$ are contained in the view image of
$\inst_2$, $Q$ holds in $\inst_1$ but not in $\inst_2$.  And we can check
that they are counterexamples effectively -- in fact, even efficiently. We simply check that the rules hold, compute
the view images, and compute the query results.
Therefore, the finite variants of the problems we consider are always co-computably enumerable (co - c.e).
Recall that problems that are both c.e. and co-c.e. are decidable.
Since we know that all variants of these problems  can be undecidable, in the undecidable cases
the finite variants must fail to be  c.e.

We mentioned in the conclusion of the paper that monotonic determinacy with rules over all instances
can be ``worse than undecidable'', in the following sense:
%\michael{Check that it is mentioned}.
%michael: ok


\begin{proposition}
If $Q$ ranges over Datalog queries, $\views$ ranges over  UCQ views, $\Sigma$  over frontier-guarded
TGDs, then  monotonic determinacy over all instances is neither ce or co-ce.
\end{proposition}

\begin{proof} If the problem were c.e, the same would be true without rules.
Since without rules monotonic determinacy is finitely controllable, and since the finite variant
is always  co-c.e., this means the problem is co-c.e. Thus, if the problem were c.e. it would be decidable.
But we know \cite{uspods20journal} the problem of monotonic determinacy without rules
is undecidable for general Datalog queries and UCQ views, which is a contradiction.


Now suppose the problem were co-c.e.  Then the same would be true for $Q$ a CQ. 
But if $Q$, $\Sigma$,  and $\views$ are all first-order, the problem is always c.e., since we have proofs of the corresponding entailment as a witness.
So if the problem were co-c.e. it would be decidable. Thus we would conclude that monotonic
determinacy for $\fgtgd$ rules, CQ queries, and  UCQ views is decidable. This is a contradiction given that we have shown
even special cases of this problem are undecidable: see, e.g. Theorem \ref{thm:undecfrontonepluslinearcqboth}.
\end{proof}



==> problematiccert.tex <==

Recall the statement of Theorem
 \ref{thm:autpre} [Automata for entailing witnesses] 

\medskip

Let $\Sigma$ consist of frontier-guarded TGDs, $\views$ a set of views defined
by $\fgdl$ Datalog queries, and $Q$ a $\fgdl$ query.
Let $k$ be a number.

There is a tree automaton $T_{Q, \views, \Sigma, k}$ that runs over $k$-tree codes in the view signature
such that for every finite $\vinst_0$ of tree-width $k$,


$T_{Q, \views, \Sigma, k}$ accepts a code of $\vinst_0$ if and only if $\vinst_0 \models_{\views, \Sigma} Q$.

\medskip

\begin{proof}
By Lemma~\ref{lem:datalog to ucq} it suffices to consider the case where
the views in $\view$ are UCQs.



We are going to define a MSO formula $\psi$ for the schema
of $\codes{(\viewschema)}{k}$-trees such that for every
$\codes{(\viewschema)}{k}$-tree $\tree$ we have that $\tree \models
\psi$ iff $\tree$ is a tree code and $\inst \models
\varphi$ for all $\inst \in \viewback(\decode{\tree})$. The statement of
the proposition then follows, because finite tree automata can
capture any MSO property. It is clear that there is a MSO formula $\tau$
(or an automaton) that expresses that $\tree$ is a tree code. Thus, it
suffices to define an MSO formula $\beta$ such that for all tree codes
$\tree$
\begin{equation} \label{e:target formula}
 \tree \models \beta \iff \inst \models \varphi \mbox{ for all } \inst
\in \viewback(\decode{\tree}), 
\end{equation}
and then just set $\psi = \tau \land \beta$.

The main difficulty is to express the quantification over all approximations
in the right hand side of \eqref{e:target formula} with monadic
quantifiers over the tree $\tree$. The proof strategy is to extend the
bags that are encoded at the nodes of $\tree$ with additional local
names that hold of the approximations of any of the view facts in the bag. To
this aim we define a notion of extended tree codes, which are tree codes
for the schema $\schema' = \viewschema \uplus \schema$ that are supposed
to represent the view instance $\decode{\tree}$, together with one of
its approximations $\inst \in \viewback(\decode{\tree})$. We provide more
details in the paragraphs below.

For every UCQ $\view_i$ in $\view$ let $a_i$ denote its arity. For every
UCQ $\view_i$ in $\view$ let $R_i$ be the finite set of all canonical
instances of the CQs in the UCQ $\view_i$. Each of the instances $\rinst
\in R_i$ can be seen as an instance for the schema $\schema_i$, which
extends the schema $\schema$ of $\varphi$ with additional constants
$c_1,\dots,c_{a_i}$, that mark the positions of the answer variables of
$\view_i$.

Let $b$ be  the maximal size of any of the $\rinst \in R_i$ for any
$i$ and set $k' = k + r \cdot (k + 1)^m \cdot b$, where $r$ is the
number of views in $\view$ and $m$ is the maximal arity of any of the
views in $\view$. It is clear that for every view $\view_i$ in $\view$,
any approximation instance $\rinst \in R_i$,  and any tuple $\ntuple =
(l_1,\dots,l_{a_i})$, there is an injective function
$e^\rinst_{i,\ntuple}$ from the domain of $\rinst$ to $\{1,\dots,k'\}$
such that $e^\rinst_{i,\ntuple}(c_j) = l_i$, meaning that the element
corresponding to the $j$-th answer variable in $\rinst$ is mapped to the
$j$-th element in the tuple $\ntuple$. The number $k'$ is chosen large
enough to ensure that the approximations of any view
facts overlap only at their answer variables. Formally, this means that
for all views $\view_i$ and $\view_{i'}$ in $\view$, $\ntuple =
(l_1,\dots,l_{a_i})$ and $\ntuple' = (l'_1,\dots,l'_{a_{i'}})$ such that
either $\view_i \neq \view_{i'}$ or $\ntuple \neq \ntuple'$, and
moreover, for all $\rinst \in R_i$, $\rinst' \in R_{i'}$, with elements
$a$ from $\rinst$ and $a'$ from $\rinst'$ such that $a$ is not answer
variable of $\rinst$ and $a'$ is not an answer variable of $\rinst'$, it
holds that $e^\rinst_{i,\ntuple}(a) \neq e^{\rinst'}_{i',\ntuple'}(a')$.

Define an \emph{extended tree code} to be a
$\codes{(\schema')}{k'}$-tree such that:
\begin{enumerate}
 \item \label{i:tree code} The tree $\tree$ is a
$\codes{(\schema')}{k'}$-tree code 
 \item \label{i:extension is local} For every $T_g$ that is true at a
vertex $v$ of $\tree$ the partial injection $g$ is such that its domain
and range are both contained in $\{1,\dots,k\}$.
 \item \label{i:no equality in extension} If $T^{=}_{l,l'}$ is true at a vertex $v$ of $\tree$ then $l,l'
\leq k$.
 \item \label{i:no view facts in extension} If $T^{\view_i}_\ntuple$ is
true at a vertex $v$ of $\tree$ for some view symbol $\view_i$ from
$\viewschema$ then $\ntuple \in \{1,\dots,k\}^{a_i}$, that is, $\ntuple$
contains only local names from $\{1,\dots,k\}$.
 \item \label{i:unfoldings are there} For every vertex $v$ of $\tree$
there is a function $\upsilon_v$ that maps any pair $(\view_i,\ntuple)$,
where $T^{\view_i}_\ntuple$ is true at a vertex $v$, to an element
$\upsilon_v(\view_i,\ntuple) \in R_i$ such that
\begin{enumerate}
 \item for every fact $R(b_1,\dots,b_h)$ in $\rinst =
\upsilon_v(\view_i,\ntuple)$ such that $T^{\view_i}_\ntuple$ is true at
$v$ the predicate $T^R_\mtuple$ is true at $v$ for $\mtuple =
(e^\rinst_{i,\ntuple}(b_1),\dots,e^\rinst_{i,\ntuple}(b_h))$, and
 \item if $T^R_\mtuple$ is true at $v$ then there is some
$T^{\view_i}_\ntuple$ that is true at $v$ and a fact $R(b_1,\dots,b_h)$
in $\rinst = \upsilon_v(\view_i,\ntuple)$ such that $\mtuple =
(e^\rinst_{i,\ntuple}(b_1),\dots,e^\rinst_{i,\ntuple}(b_h))$.
\end{enumerate}
\end{enumerate}
One can check that there is an MSO formula $\eta$ such that $\tree
\models \eta$ iff $\tree$ is an extended tree code.

\michael{This needs an overhaul: the ``proof text'' amounts
to  restating what we want to prove rather than proving it}

Every $\codes{(\schema')}{k'}$-tree $\tree$ projects to a
$\codes{\schema}{k'}$-tree $\restr{\tree}{\schema,k'}$ if we
just forget all the predicates of the form $T^{\view_i}_\ntuple$ for
some view relation $\view_i$ in $\view$. Moreover, it is obvious that if
$\tree$ is a $\codes{(\schema')}{k'}$-tree code then its projection
$\restr{\tree}{\schema,k'}$ is a $\codes{\schema}{k'}$-tree
code.

Similarly, every $\codes{(\schema')}{k'}$-tree $\tree$ projects to a
$\codes{(\viewschema)}{k}$-tree $\restr{\tree}{\viewschema,k}$. We just
forget all the predicates that mention any local name $l > k$ or that
are of the form $T^R_\ntuple$ for some relation symbols $R$ from
$\schema$. Because of items \ref{i:tree code}, \ref{i:extension is
local} and \ref{i:no equality in extension} above we have that if
$\tree$ is an extended tree code then $\restr{\tree}{\viewschema,k}$ is
a $\codes{\viewschema}{k}$-tree code.

Extended tree codes capture the backwards mapping of views. This is
made precise by the following two properties of extended tree codes:
\begin{description}
 \item[Soundness:] For every extended tree code $\tree$ there is an $\inst \in
\viewback(\decode{\restr{\tree}{\viewschema,k}})$ such that $\inst \cong
\decode{\restr{\tree}{\schema,k'}}$.
 \item[Completeness:] For every $\codes{(\viewschema)}{k}$-tree code $\tree'$ and
$\inst \in \viewback(\decode{\tree'})$ there is an extended tree code
$\tree$ such that $\restr{\tree}{\viewschema,k} = \tree'$ and
$\decode{\restr{\tree}{\schema,k'}} \cong \inst$.
\end{description}
Using items \ref{i:no view facts in extension} and \ref{i:unfoldings are
there} from the definition of extended tree codes, one can check that
these properties hold.

We then also observe that in MSO we can evaluate GSO formulas over the
models that are encoded over tree codes. Thus, there is an MSO formula
$\varphi'$ such that for all $\codes{\schema}{k'}$-tree codes $\tree$
\[
 \tree \models \varphi' \iff \decode{\tree} \models \varphi .
\]
This is quite obvious. %Either one just believes it, or 
One can see this  using
Proposition~\ref{prop:fmltoaut} and the fact that tree automata can be
translated to MSO. Also note that the only difference between
$\codes{\schema}{k'}$ and $\codes{(\schema')}{k'}$ are that the latter
contains additional predicate symbols. Hence, the formula $\varphi'$
can also be evaluated over extended tree codes $\tree$ for which we have
that
\[
 \tree \models \varphi' \iff \decode{\restr{\tree}{\schema,k'}} \models
\varphi .
\]

Define the MSO formula $\beta$ as follows:
\[
 \beta \equiv \forall Q_1\dots\forall Q_s (\eta \rightarrow \varphi'),
\]
where $Q_1,\dots,Q_s$ are all the predicate symbols that are in
$\codes{\schema}{k'}$. The idea on a $\codes{(\viewschema)}{k}$ tree is to
consider all extensions to a $\codes{(\schema')}{k'}$-tree, which need to
extended tree codes because of $\eta$, and then make sure that they all
satisfy $\varphi$. By the soundness and completeness properties of extended
tree codes it follows that this definition of $\beta$ satisfies
\eqref{e:target formula}.
\end{proof}




==> tentaclestuff.tex <==
\subsection{Extensions with monadic tentacles} \label{subsec:extension}



\begin{definition}
 A structure $\estruct$ is a \emph{monadic tentacle extension} of
$\struct$ if $\struct \subseteq \estruct$ and
for every element $a$ in $\struct$ there is a pointed structure
$(\estruct_a,r_a)$ such that $\estruct$ is obtained from $\struct$ by
adding all the facts $\estruct_a$ for $a$ in $\struct$, and then identifying
$r_a$ from $\estruct$ with $a$ from $\struct$.
\end{definition}

\begin{theorem} \label{thm:tentacleextension}
 For every $n$ there is a $k$ such if $\struct \equiv_k \struct'$ for
some structures $\struct$ and $\struct'$ then for every monadic tentacle
extension $\estruct$ of $\struct$ there is a monadic tentacle extension
$\estruct'$ of $\struct'$ such that $\estruct \equiv_n \estruct'$.
\end{theorem}
\begin{proof}
Fix $n$. Let $t$ be the number of $\equiv_n$-types and set $k = (n + 1)
\cdot t + 1$
% types of pointed structures or of structures?
Let $\struct$ and $\struct'$ be two structures such that $\struct
\equiv_k \struct'$.

Consider a monadic tentacle extension $\estruct$ of $\struct$, which is
given by tentacles $(\estruct_a,r_a)$ for all $a$ in $\struct$.
Partition the elements of $\struct$ into sets $T_1,\dots,T_h$, which are
the $\equiv_n$-equivalence classes of their tentacles in
$\estruct$. Thus, for every $i \in \{1,\dots,h\}$ there is some $a_i$ in
$\struct$ such that
\[
 T_i = \{b \mid b \mbox{ is in } \struct \mbox{ and } (\estruct_b,b)
\equiv_n (\estruct_{a_i},a_i)\} .
\]
The number $h$ is bound by the number $t$ of $n$-types.

We then consider what happens when Spoiler plays the sets
$T_1,\dots,T_h$ in successive rounds in a match against Spoilers winning
strategy in $\struct \equiv_k \struct'$. Let the subsets
$T'_1,\dots,T'_h$ of $\struct'$ be the replies by Duplicator. These
$T'_1,\dots,T'_h$ partition the elements in $\struct'$, because otherwise
Spoiler could use one of the additional rounds that are left afterwards
to win.

We define the tentacle extension $\estruct'$ of $\struct'$ such that for
every $a' \in T'_i$ in $\struct'$ we attach the structure
$(\estruct_{a_i},a_i)$ as a tentacle at $a'$. For every $a' \in T'_i$
let $(\estruct'_{a'},a')$ be the structure $(\estruct_{a_i},a_i)$, where
we identify $a'$ with $a_i$. Thus, $\struct'$ is the is the tentacle
extension of $\struct'$ with the tentacles $(\estruct'_{a'},a')$ for all
$a'$ in $\struct'$.

We need to construct a winning strategy for Duplicator that shows that
$\estruct \equiv_n \estruct'$. The inductive invariant for defining this
strategy is as follows: Assume that we have already played a match $m_E$
in the game for $\estruct \equiv_n \estruct'$ on which the sets
$(P_1,P'_1),\dots,(P_h,P'_h)$ and the points
$(e_1,e'_1),\dots,(e_o,e'_o)$ have been played and in $l$ rounds are
left to be played. Then there is a shadow match $m_B$ in the game for
$\struct \equiv_k \struct'$, where Duplicator plays according to her
winning strategy, at least $l \cdot t$ rounds are left to play and the
following conditions are satisfied:
\begin{enumerate}
 \item \label{i:tentacle matches} For each pair $(b,b')$ that has been
played in $m_B$ there is a shadow match $m_{b,b'}$ that is played
according to Duplicators winning strategy for $(\estruct_b,b) \equiv_n
(\estruct'_{b'},b')$, on which the restrictions of
$(P_1,P'_1),\dots,(P_h,P'_h)$ to the structures $\estruct_b$ and
$\estruct'_{b'}$ have been played and there are at least $l$ rounds are
left to play.
 \item \label{i:move to base} For each $(e,e')$ that has been played in
$m_E$ there is a $(b,b')$ that has been played on $m_B$ such that $e$ is
in $E_b$ and $e'$ is in $E_{b'}$ and $(e,e')$ has been played on
$m_{b,b'}$. (This also allows for the case where $(b,b') = (e,e')$.)
 \item \label{i:types} There are $(T_1,T'_1),\dots,(T_h,T'_h)$ that have
been played in $m_B$ such that
\begin{enumerate}
 \item the sets $T_1,\dots,T_h$ partition the domain of $\struct$,
 \item the sets $T'_1,\dots,T'_h$ partition the domain of $\struct'$, and
 \item for all $j \in \{1,\dots,h\}$, $b \in T_j$ and $b' \in T'_j$ we
have 
\[
 (\estruct_b,b,P_1,\dots,P_h) \equiv_l
(\estruct'_{b'},b',P'_1,\dots,P'_h).
\]
(Here, we just write $P_1,\dots,P_h$, but mean the restrictions of these
sets to the domain of the structure $\estruct_b$, and similarly for
$P'_1,\dots,P'_h$ and $\estruct'_{b'}$.)
\end{enumerate}
\end{enumerate}

We first show that these conditions can be guaranteed at the start of
the match $m_E$. At the beginning of the match $m_E$ we let shadow match
$m_B$ be the match which is played according to Duplicator's winning
strategy in the game for $\struct \equiv_k \struct'$, where the sets
$(T_1,T'_1),\dots,(T_h,T'_h)$ that are used to define the extension
$\estruct'$ above have already been played. Because $h$ is smaller than
$t$, $k = (n + 1) \cdot t$ and $l = n$ there are then still at least $l
\cdot t$ rounds left to be played on $m_B$. Conditions \ref{i:tentacle
matches} and \ref{i:move to base} are trivially satisfied because so far
no pairs of elements have been played on the matches $m_B$ and $m_E$.
The construction of $\estruct'$ guarantees that condition~\ref{i:types}
is satisfied at the beginning of the game.

\medskip

We then show that Duplicator can play in such a way that the invariant is
maintained. We have to consider two cases corresponding to the possible
moves of Spoiler at the beginning of the next round. Note that because
the conditions are completely symmetric it suffices to consider the case
where Spoiler moves in $\estruct$.

If Spoiler chooses an element $e$ in $\estruct$ we let Duplicator reply
as follows: Let $b$ in $\struct$ be such that $e$ is in the tentacle
$\struct_b$ at $b$. This also works for the elements $e$ from $\struct$
because these are trivially in their own tentacle $\estruct_e$. We then
let $b'$ be the reply of Duplicator in the shadow match $m_b$ if Spoiler
plays $b$. We then consider the shadow match $m_{b,b'}$. If $(b,b')$ has
already been played on $m_B$ then this match already exists. Otherwise,
we use condition~\ref{i:types} to start a new shadow match $m_{b,b'}$
that satisfies condition~\ref{i:tentacle matches}. This is possible
because there must be some $i$ such that $b \in T_i$ and $b' \in T'_i$
because otherwise Duplicator would loose immediately on $m_B$ as
$(b,b')$ and all the mutual pairs of the partitions $T_1,\dots,T_h$ and
$T'_1,\dots,T'_h$ have already been played. We then see how Duplicator
replies to the move $e$ in the shadow match $m_{b,b'}$. Let $e'$ be the
reply. We let Duplicator play this $e'$ in the match $m_E$. It is easy
to check that this maintains conditions \ref{i:tentacle matches} and
\ref{i:move to base}. Condition~\ref{i:types} is trivially maintained.

In the other case Spoiler chooses to play a subset $P$ of the domain of
$E_a$. We the first use this $P$ to construct a refinement
$S_1,\dots,S_g$ of the partition $T_1,\dots,T_h$ that exists by
condition~\ref{i:types}. The idea is to let $P$ be additional structure
in the definition of $l$ types. More precisely, we choose the partition
such that for every $i \in \{1,\dots,g\}$ there is some $a_g$ such that
\[
 S_j = \{b \mid b \mbox{ is in } M \mbox{ and }
(\estruct_b,b,P_1,\dots,P_h,P) \equiv_{l - 1}
(\estruct_{a_i},a_i,P_1,\dots,P_h,P)\}.
\]
The number $g$ is bound by $t$ because of the general fact that
$(\struct,a,P_1,\dots,P_v) \equiv_{u + 1} (\struct',a',P'_1,\dots,P'_v)$
entails $(\struct,a,P_1,\dots,P_v,P_{v + 1}) \equiv_u
(\struct',a',P'_1,\dots,P'_v,P'_{v + 1})$. Because of this fact it is
also the case that $S_1,\dots,S_g$ refines $T_1,\dots,T_h$.

We then let Spoiler play the sets $S_1,\dots,S_g$ in the shadow game
$m_B$ and let $S'_1,\dots,S'_g$ be the replies of Duplicator, playing
her winning strategy. The sets $S'_1,\dots,S'_g$ partition the domain of
$\struct'$ and this partition refines $T'_1,\dots,T'_h$. Otherwise,
Spoiler could use the remaining round to win in $m_B$. To define the
reply $P'$ of Duplicator in $m_E$ we consider all tentacles separately.
Thus, fix some $b'$ in $\struct'$. If there is already a pair $(b,b')$
that has been played in $m_B$ then let $P'_{b'}$ be the reply of
Duplicator in the shadow match $m_{b,b'}$ if Spoiler plays the
restriction of $P$ to the domain of $\estruct_b$. This is well-defined
because $(b,b')$ is played on a match where Duplicator plays a winning
strategy and hence $b$ is unique. If $b'$ has not yet occurred on $m_B$
then let $i$ be such that $b' \in S'_i$ and define $P'_{b'}$ be such
that
\[
 (\estruct_{a_i},a_i,P_1,\dots,P_h,P) \equiv_{l - 1}
(\estruct'_{b'},b',P'_1,\dots,P'_h,P'_{b'}),
\]
where $a_i$ is the representative that was mentioned in the definition
of $S_i$. Such a $P'_{b'}$ must exist because the $S$-partitions refine
the $T$-partitions and by condition~\ref{i:types} we then have that
\[
 (\estruct_{a_i},a_i,P_1,\dots,P_h) \equiv_l
(\estruct'_{b'},b',P'_1,\dots,P'_h).
\]
This concludes the definition of $P'_{b'}$ for an arbitrary $b'$ in
$\struct'$. We then set $P' = \bigcup \{P'_{b'} \mid b' \mbox{ in }
\struct'\}$ and let Duplicator reply with $P'$ in $m_E$. Trivially, this
maintains condition~\ref{i:move to base} and it is quite easy to see
from our definition of $P'_{b'}$ that it also preserves
condition~\ref{i:tentacle matches}. We have also already argued that the
first two parts of condition~\ref{i:types} are satisfied. To prove the
last part of condition~\ref{i:types} it suffices because of the
definition of $S_j$, and the transitivity of $\equiv_{l - 1}$, that we
show that $(\estruct_{a_i},a_i,P_1,\dots,P_h,P) \equiv_{l - 1}
(\estruct'_{b'},b',P'_1,\dots,P'_h,P'_{b'})$ for all $b' \in S'_j$. If
there is no tuple $(b,b')$ that has been played on $m_B$ then this
follows immediately from the definition of $P_{b'} \subseteq P$. If
$(b,b')$ occurs on the match $m_B$ then we consider the shadow match
$m_{b,b'}$. By condition~\ref{i:tentacle matches} the restrictions of
the pairs $(P_1,P'_1),\dots,(P_h,P'_h)$ have been played up to the start
of the current round and in the current round we add the restriction of
the pair $(P,P')$. Because there are still $l-1$ round to be played and
Builder is playing according to a winning strategy this means that
$(\estruct_b,b,P_1,\dots,P_h,P) \equiv_{l - 1}
(\estruct'_{b'},b',P'_1,\dots,P'_h,P'_{b'})$. Because $b' \in S_i$ it
follows that $b \in S_i$, otherwise Duplicator could not win the match
$m_B$. Thus, it follows from the definition of $S_i$ that
$(\estruct_{a_i},a_i,P_1,\dots,P_h,P) \equiv_{l - 1}
(\estruct_b,b,P_1,\dots,P_h,P)$. With the transitivity of $\equiv_{l -
1}$ we obtain that required $(\estruct_{a_i},a_i,P_1,\dots,P_h,P)
\equiv_{l - 1} (\estruct'_{b'},b',P'_1,\dots,P'_h,P'_{b'})$.

\medskip

Lastly, we argue that Duplicator wins the match $m_E$. Let $I$ be the
set of pairs $(e,e')$ that are played at the end of the game after
$n$-rounds when, $l = 0$. Because by condition~\ref{i:move to base} all
the pairs $(e,e')$ that are played on $m_E$ occur in one of the shadow
matches $m_{b,b'}$, and these shadow matches do not overlap, it is clear
that that $I$ is a partial bijection.

To show that $I$ preserves the interpretation of relation symbols it
suffices because of symmetry to show the preservation in one direction.
Before we do so we make the following observation about tuples
$\tuple{e} = (e_1,\dots,e_i)$ of elements from $\estruct$ that are in
the domain of $I$, meaning that there is a tuple $\tuple{e}' =
(e'_1,\dots,e'_i)$ such that $(e_1,e'_1),\dots,(e_i,e'_i) \in I$:
\begin{enumerate}
 \item If $\tuple{e}$ is not empty and all its element are in some
tentacle $(\estruct_b,b)$ of $\estruct$ then there is a $b'$ in
$\struct'$ such that $e'_1,\dots,e'_i$ are in the tentacle
$(\estruct'_{b'},b')$ and the pairs $(e_1,e'_1),\dots,(e_i,e'_i)$ are
played on $m_{b,b'}$.
 \item If all elements $e_1,\dots,e_i$ are all in $\struct$
then the elements $e'_1,\dots,e'_i$ are all in $\struct'$ and the pairs
$(e_1,e'_1),\dots,(e_i,e'_i)$ are played on $m_B$.
\end{enumerate}
The first of this items holds because a suitable $b'$ exists by
condition~\ref{i:move to base} and it must be the same for all the
$e_1,\dots,e_2$ because the pairs played on $m_B$ are a partial
bijection. To see that the second of these items holds observe that if
$(e,e')$ is played on $m_E$ and $e$ is in $\struct$ then $e$ must be
equal the base point $b$ of the tentacle $(\estruct_b,b)$ such that $e$
is in $\estruct_b$, which exists by condition~\ref{i:move to base}.


To see that $I$ preserves the interpretation of the relations symbols in
$\estruct$ consider any tuple $\tuple{e}$ of elements in $\estruct$ that
is in the interpretation of some relation symbol $R$, such that all
elements in $\tuple{e}$ are in the domain of $I$. By the definition of
the monadic tentacle extension this means that $\tuple{e}$ is already in
the interpretation of $R$ at $\struct$ or it is in the interpretation of
$R$ at one of the tentacle.

We first consider the case where $\tuple{e}$ is in the interpretation of
$R$ at some tentacle $(\estruct_b,b)$ for $b \in T_i$. In the special
case where $\tuple{e}$ is empty we can consider any $b' \in T'_i$ and
then $R$ must be true at the tentacle $(\estruct'_{b'},b')$ of
$\estruct'$ because of condition~\ref{i:types}. In the other case where
$\tuple{e} = (e_1,\dots,e_i)$ is not empty we consider the pairs
$(e_1,e'_1),\dots,(e_i,e'_i) \in I$. By the item above there is some
$b'$ in $\struct'$ such that $e'_1,\dots,e'_i$ all occur in the tentacle
$(\struct'_{b'},b')$ and all $(e_1,e'_1),\dots,(e_i,e'_i)$ are played on
$m_{b,b'}$. Because $m_{b,b'}$ is winning for Duplicator the pairs
played on $m_{b,b'}$ result in a partial isomorphism between the
tentacles $(\estruct_b,b)$ and $(\estruct'_{b'},b')$. It follows that
$\tuple{e}'$ is in the interpretation of $R$ at $(\estruct'_{b'},b')$
and hence also at $\estruct'$.

In the other case $\tuple{e}$ is in the interpretation of $R$ in
$\struct$. Because by the second item above the pairs
$(e_1,e'_1),\dots,(e_i,e'_i)$ are played on $m_B$, and this match is
winning for Duplicator, it follows that $\tuple{e}'$ is in the
interpretation of $R$ at $\struct$.

To check that $I$ preserves all the monadic predicates that have been
played on $m_E$ consider any pair of elements $(e,e')$ and pair of sets
$(P,P')$ that have been played on $m_E$. By condition~\ref{i:move to
base} $(e,e')$ is also played on one of the shadow matches $m_{b,b'}$.
And, by condition~\ref{i:tentacle matches} the restrictions of the pair
$(P,P')$ to the tentacles $(\estruct_b,b)$ and $(\estruct'_{b'},b')$ is
played. But because this match is winning for Duplicator it follows from
$e \in P$ that $e' \in P'$. The proof of preservation in the direction
from $\estruct'$ to $\estruct'$ is analogous.
\end{proof}



==> treecodes.tex <==




\myparagraph{Tree codes}
We will now discuss how to represent tree decompositions by labeled
trees called tree codes. There are a number of ways to code in the prior literature.
See, for example Appendix A.1 of \cite{visible}. Our encoding will be more verbose
than many prior ones, using two kinds of node labels. We do this to make one of our later
transformations (the ``backward mapping'' of Proposition \ref{prop:backward}) simpler.

Given a schema $\aschema$ we derive from it a schema $\sigcode{\aschema}{k}$ in the following way:
\begin{compactitem}
\item for every relation $R \in \aschema$ of arity $m$ and every sequence $\vec{n} = n_1, \dots, n_m$ of 
numbers less than or equal to $k$
there is a unary relation $\coderel^R_{\vec{n}}$ in $\sigcode{\aschema}{k}$.

\item for every partial 1-1 map $\ssuper$ from $\{1, \dots, k\}$ to $\{1, \dots, k\}$, there is a unary relation
$\coderel_\ssuper$. 
\end{compactitem}

A \emph{tree code} $\T$ (\emph{of width} $k$) is a rooted tree with its nodes labeled with symbols from 
$\sigcode{\aschema}{k}$. Each non-root node can be labelled with multiple symbols of the form $\coderel^R_{\vec{n}}$ and exactly one symbol of the form $\coderel_\ssuper$. A root node can only have labels of the form $\coderel^R_{\vec{n}}$. 
For a node $n$ we will write $A(n)$ to denote that $n$ is labelled with symbol $A$. 
We will call any natural number in $\{1 \ldots k\}$ a \emph{local name}. One can view tree codes as instances over $\sigcode{\aschema}{k} \cup \{E\}$ where $E$ is some fixed edge relation symbol.

Given an instance $\inst$ any of its tree decompositions $(\tau, \lambda)$ gives a rise to a tree code $\T$ in a following way. The underlying tree of $\T$ is $\tau$. Let $v$ be a non-root node of $\tau$ such that $\lambda(v) = (b_1, \ldots, b_k)$ and let $u$ be a parent of $v$ such that $\lambda(u) = (a_1, \ldots a_k)$ then $v$ is labelled in $\T$ with $\coderel_\ssuper$ where $\ssuper = \{ (i,j) | a_i = b_j\}$. Moreover, for every atom $R(b_{n_1}, \dots b_{n_m}) \in \inst$ there exists at least one node $v$ in $\T$ such that $\lambda(v) = (b_1, \ldots, b_k)$ and that $\coderel^R_{n_1, \ldots n_m}$ is a label of $v$ in $\T$ In such case we will say that $\T$ \emph{encodes} $(\tau, \lambda)$. Note that for some tree decompositions there might exist more than one such tree code.



A \emph{decoding} of $\T$, denoted $\decode{\T}$, is the $\aschema$ instance created as follows:
Define an binary relation $\equiv_0$ on $\adom(\T) \times [1,k]$ by stating that $(u,i) \equiv_0 (v,j)$ 
if $u$ is the parent of $v$ and there exists a label $\coderel_\ssuper$ of $v$ such that $\ssuper(i)=j$. Let $[u,i]$ denote the equivalence class of $(u,i)$ in an equivalence relation generated by $\equiv_0$. Then $R([u,n_1], \ldots [u,n_m])$ is an element of $\decode{\T}$ if and only if there exists a node $u$ of $\T$ such that $\coderel^R_{n_1, \ldots n_m}$ is a label of $u$.


From the above definition it is clear that if we have a tree decomposition, the
corresponding tree codes contain all the information encoded
in the instance being decomposed:

\begin{proposition}\label{prop:encode-decode}
Let $\inst$ be an instance,  $(\tau, \lambda)$ be a tree decomposition, and $\T$ a tree code encoding
$(\tau, \lambda)$. 
Then $\decode{\T}$ is isomorphic with $\inst$.
\end{proposition}

Moreover, one can reorganize local names of any given tree code to get:
\begin{proposition}\label{prop:tree-code-id}
Let $\T$ be a tree code then there exists a tree code $\T'$ such that $\decode{\T}$ is isomorphic to $\decode{\T'}$ and that every partial mapping $\ssuper$ in any $\coderel_\ssuper$ label of $\T'$ is an identity.
\end{proposition}

We want the tree codes to be read by a tree automaton, which work on trees
which each node has a single label.  To this end, 
we will treat the set of fact and partial-function labels as a single label $\sigma_L^{\ssuper}$, where $L$ is a collection of 
$\coderel^R_{\vec{n}}$ symbols and $\ssuper$ enumerates pairs that give the partial function. 
We will sometimes abuse notation by treating $\sigcode{\aschema}{k}$ as the consolidated
label alphabet for a tree automaton.
And when we do not need to make explicit the vocabulary $\sigcode{\aschema}{k}$ of predicates that we compress in
this way, we will abbreviate the set of $\sigma_L^{\ssuper}$ symbols with $\TreeAlphabet$.

\begin{example}\label{ex:tree-codes}
An example of  an instance $\inst$  and a tree decomposition $\TD$ of $\inst$
are shown  on the left side of  Figure~\ref{fig:tree-codes-example}. 
Continuing to the right we have The tree code $\T$ corresponding to  $\TD$,
 and its decoding $\decode{\T}$. Note that the decoding is isomorphic to the original
instance $\inst$.
\begin{figure}  
    \centering
    \includegraphics{example-figures/tree-codes-example}
    \caption{From left to right: an instance, a tree decomposition of the instance,
a tree code, and its decoding (isomorphic to the instance)}
 \label{fig:tree-codes-example}
\end{figure}
\end{example}




